Optimal Control for Linear Networked Control Systems with Information Transmission Constraints

This paper addresses the problem of robust control of a linear discrete-time system subject to bounded disturbances and to measurement and control budget constraints. Using Q-parameterization and a polytope containment method, we prove that the co-design of an affine feedback controller, a measurement schedule and a control schedule can be exactly formulated as a mixed integer linear program with 2 binary variables per time step. As a consequence, this problem can be solved efficiently, even when an exhaustive search for measurement and control times would have been impossible in a reasonable amount of time.

==> appendices/solution_properties.tex <==
\section{Properties of the Solution} \label{subsec:properties}

\KR{A polytope $\mathcal{P} \subseteq \R^{n}$ is \emph{full-dimensional} if there exists an element $p\in\mathcal{P}$ and a radius $r>0$ such that $\{ x \in \R^n \; | \; \| p - x \| \leq r \} \subseteq \mathcal{P}$.}

There were many possible constraints considered and solution methods proposed for Problem \ref{prob:control_asap}. In this section, we analyze some of those proposals and discuss the reasoning behind why they could be considered and what advantages they provide in the synthesis for problems like Problem \ref{prob:control_asap}.

\subsubsection{Constraints on the Measurement Signal $\modeSymbol^m$}

The property of observability (or detectability) of a system is one of the fundamental constraints which determines the feasibility of Problem \ref{prob:control_asap} (similarly, observability determines the objective value of \ref{prob:control_alap}). In the measurement scheduling problem, this property can be analyzed using the methods of \cite{jungers2018observability}. An observability matrix can be defined for the system in \ref{eq:system_w_missing_meas} as follows:

\begin{definition}[Observability Matrix $\mathcal{O}_{\sigma^m}$ \cite{jungers2018observability}]
    Given a measurement signal $\modeSymbol^m$, the \emph{observability matrix} of the system \eqref{eq:system_w_missing_meas} at time $t$ is:
    \begin{equation*}
        \mathcal{O}_{\sigma^m}(t) =
        \begin{bmatrix}
            \modeSymbol^m_0 C \\
            \modeSymbol^m_1 CA \\
            \vdots \\
            \modeSymbol^m_{t-1} CA^{t-1}
        \end{bmatrix}\in \mathbb{R}^{(t+1)n_y \times n_x}.
    \end{equation*}
\end{definition}

The null space of this matrix can be analagously called the unobservable space of initial conditions for system \eqref{eq:system_w_missing_meas} when no noise is present. Intuitively, the choice of measurement times is determining the unobservable initial conditions of the system and should somehow incorporate information about which initial conditions may violate our constraints on the output $z_t$.

Now, consider the set of initial conditions which \emph{escape} the performance constraint at time $T$:
$$
\EscapeSetFromXatT =
\left \{
    x_0 \in \mathcal{X}_0 
    \; | \;
    \exists \{ w_\tau \}_{\tau=0}^{T-1} \text{ s.t. } z_T^{(ol)} \notin \performanceSet
\right \}.
$$
where the open loop performance output at time $T$, $z_T^{(ol)}= D ( A^{T} x_0)+d$, is a linear function of $x_0$. The variable $z_T^{(ol)}$ can also be redefined as $z_T^{(ol)}= D ( A^{T} x_0 + \sum_{\tau=0}^{T-1} A^{T-1-\tau} w_\tau)+d$ with $w_\tau$ being parallel to $x_0$, but we omit this more general definition for clarity of the exposition.

A relationship between $\mathcal{O}_{\sigma^m}(T)$ and $\EscapeSetFromXatT$ can then be used to define an overapproximation of the feasible set of solutions to Problem \ref{prob:control_asap}:

\begin{proposition}
    \label{prop:observability_of_optimal_sigma}
    Consider the safety problem (Problem \ref{prob:control_asap}) with sets $\mathcal{W},\V,\performanceSet$ being symmetric about the origin and $d=0$ along with the set $\EscapeSetFromXatT$ with respect to the dynamics in \ref{eq:system_w_missing_meas}. The problem is feasible for $ T^* \geq T$ only if there exists a measurement signal $\sigma^m \in \zeroOneSet^{T}$ such that
    $$
    \EscapeSetFromXatT 
    \cap
    \mathcal{N}( \mathcal{O}_{\sigma^m}(T) )
    = \emptyset.
    $$
\end{proposition}
% \begin{proof}
%     Suppose that for any arbitrary choice of $\modeSymbol^m$, there exists an initial state 
%     $x_0^* \in
%     \tilde{\mathcal{X}}_0(T) 
%     \cap
%     \mathcal{N}( \mathcal{O}_{\sigma^m}(T) )
%     $.
%     By symmetry, this implies that  $-x_0^* \in \tilde{\mathcal{X}}_0(T)$ and $DA^Tx_0, -DA^T x_0 \notin \performanceSet.$ Then, by expanding the closed loop performance output when the disturbances are zero (e.g. $w=0,v=0$ for all $t$) one obtains
%     $$ 
%     z_T = D A^T x_0 + D \sum_{\tau = 0}^{T-1} A^{T-1-\tau} B f_\tau.
%     $$
%     The open loop controller $f_\tau=0$ and $f_{T-1} = s - D A^T x_0$ where $s \in \performanceSet$ can guarantee that $z_T \in \performanceSet$, but note that for the initial condition $-x_0$, $z_T = -2D A^T x_0 + s \notin \performanceSet$. In fact, for any open loop controller which cannot distinguish between $x_0$ and $-x_0$, we can show that one of the initial conditions will violate $z_T \in \performanceSet$.
    
%     Thus, if one cannot find a $\sigma^m$ such that $\tilde{\mathcal{X}}_0(T) \cap \mathcal{N}( \mathcal{O}_{\sigma^m}(T) )$ is empty, then there will exist an initial condition for which no open loop control can guarantee the performance variable at time $T$, $z_T$, remains within the symmetric safe set $\performanceSet$.
% \end{proof}

The proposition can be extended by considering a different definition of $\EscapeSetFromXat{T^*}$ where $z_T^{(ol)}$ is redefined as $z_T^{(ol)}= D ( A^{T} x_0 + \sum_{\tau=0}^{T-1} A^{T-1-\tau} w_\tau)+d$ with $w_\tau$ being parallel to $x_0$. % By translating $\performanceSet$, we can assume $d=0$ wlog. Is this still possible?

Proposition \ref{prop:observability_of_optimal_sigma} leads to the following corollary:
\begin{corollary}
    \label{cor:meas_schedule_feasible_set}
    For a given Problem \ref{prob:control_asap}, let $T^*$ and $(\sigma^m)^*$ be the optimal solutions of the problem and $T_1$ be the smallest time such that $\EscapeSetFromXat{T_1}$ is full dimensional. If $T_1$ exists and $T_1 \leq T^*$, then $\mathcal{O}_{(\sigma^m)^*}(T_1)$ has full rank (i.e. the system without noise is observable at time $T_1$).
\end{corollary}

This corollary explains that the solution of Problem \ref{prob:control_asap} will contain an initially observable measurement schedule, if there are enough measurements available in the budget. By applying this argument recursively, this corollary can be extended to say that all nontrivial measurement schedules must contain observable prefixes. Crucially, this corollary explains that all optimal schedules should contain an observable prefix and that adding such a constraint would reduce the search space and reduce the computation time of the solution.

\subsection{Proof of Proposition \ref{prop:observability_of_optimal_sigma}}

Suppose that for any arbitrary choice of $\modeSymbol$, there exists an initial state 
$x_0^* \in
\tilde{\mathcal{X}}_0(T) 
\cap
\mathcal{N}( \mathcal{O}_{\sigma}(T) )
$.
By symmetry, this implies that  $-x_0^* \in \tilde{\mathcal{X}}_0(T)$ and $DA^Tx_0, -DA^T x_0 \notin \performanceSet.$ Then, by expanding the closed loop performance output when the disturbances are zero (e.g. $w=0,v=0$ for all $t$) one obtains
$$ 
z_T = D A^T x_0 + D \sum_{\tau = 0}^{T-1} A^{T-1-\tau} B f_\tau.
$$
The open loop controller $f_\tau=0$ and $f_{T-1} = s - D A^T x_0$ where $s \in \performanceSet$ can guarantee that $z_T \in \performanceSet$, but note that for the initial condition $-x_0$, $z_T = -2D A^T x_0 + s \notin \performanceSet$. In fact, for any open loop controller which cannot distinguish between $x_0$ and $-x_0$, we can show that one of the initial conditions will violate $z_T \in \performanceSet$.

Thus, if one cannot find a $\sigma$ such that $\tilde{\mathcal{X}}_0(T) \cap \mathcal{N}( \mathcal{O}_{\sigma}(T) )$ is empty, then there will exist an initial condition for which no open loop control can guarantee the performance variable at time $T$, $z_T$, remains within the symmetric safe set $\performanceSet$.

\subsubsection{Constraints on the Control Signal $\modeSymbol^c$}

\subsubsection{Discrete Optimality}

==> sections/Q_parametrization_old.tex <==
\AA{No $B$ here, and do not use the Theorem 2 of Kwesi's paper}

The equations for $x$ and $u$ are nonlinear in the design variables $(F,f)$ \AA{Do we speak now of the $\modeSymbol$ ?}. This would normally mean that searching for design variables that satisfy constraints like $||\xi_{t+T}||_{\infty} \leq M$ would be a nonlinear and non-convex programming problem, but we simplify the search by taking inspiration from $Q$-parameterization %in (\cite{Skaf:10}) 
and introducing the nonlinear mappings $Q \triangleq F(I-\bar{C} SF)^{-1}$ and $r \triangleq (I + Q\bar{C} S)f$. This transforms the $P$ matrix into the following:
$$
\begin{array}{rl}
	P_{x w} = & S + SQ \bar{C} S,  \ \
    P_{x v} =  SQ, \ \
    P_{u w} =  Q \bar{C} S, \ \
    P_{u v} =  Q
\end{array}
$$
and
$$
\begin{array}{rl}
	\tilde{x} = & (I+SQ\bar{C}) Jx_0 + Sr, \quad 
    \tilde{u} =  Q\bar{C} Jx_0 + r.
\end{array}
$$

These relations are linear in the design variables $Q$ and $r$. It is shown in \cite[Equations (22) and (23)]{rutledge2020finite} that this mapping is invertible and that the inverse is
\begin{align}
    \label{eq:Q_param:F}
    F&=(I+Q\bar{C}S)^{-1}Q, \\
    f&=(I+Q\bar{C}S)^{-1}r.\label{eq:Q_param:f}
\end{align}
Finally, equation (\ref{eq:closed_loop_est_error}) can be rewritten
\begin{equation*}
  \begin{bmatrix}
      x	\\	u
\end{bmatrix}
  =
  P
  \begin{bmatrix}
     w	\\	v  \\  x_0
\end{bmatrix}
  +
  \begin{bmatrix}
      Sr	\\	r
\end{bmatrix}
\end{equation*}
where
\begin{equation*}
P=
\begin{bmatrix}
     P_{x w}	&	P_{x v}  & P_{x x_0}\\
        P_{u w}	&	P_{u v}  & P_{u x_0}
\end{bmatrix}
\end{equation*}
with $P_{x w}$, $P_{x v}$, $P_{u w}$ and $P_{u v}$ defined as before and
\begin{equation*}
P_{x x_0}=(I+SQ\bar{C})J \text{\ and\ } P_{u x_0}=Q\bar{C}J. 
\end{equation*}

==> sections/estimation.tex <==
This section presents the estimation counterparts of Problems \ref{prob:control_asap} and \ref{prob:control_alap} and how to reduce these estimation problems to the control problems.

One wants to estimate the output $z_t$ of the system (\ref{eq:system_w_missing_meas}) from noisy measurements $y_\tau$ ($\tau\leq t$). To this end, we consider the following Luenberger-like estimator:
\begin{subequations}
    \label{eq:luenberger_like_estimator}
    \begin{align}
    	\label{eq:luenberger_like_estimator:x}
    	\hat{x}_{t+1} & = A \hat{x}_t + B u_t - \estFeedback_t, \\
    	\hat{y}_t & = C \hat{x}_t, \label{eq:luenberger_like_estimator:y}\\
    	\hat{z}_t&=D\hat{x}+d, \label{eq:luenberger_like_estimator:z}
    \end{align}
\end{subequations}
with feedback:
\begin{equation}
    \label{eq:affine_fb_law}
    \estFeedback_t = f_t + \sum_{\tau\leq t \text{\ s.t.\ }\modeSymbol^m_\tau=1 } F_{(t,\tau)} \bar{y}_\tau,
\end{equation}
where $\bar{y}_\tau=y_\tau-\hat{y}_\tau$.

Taken together, \eqref{eq:system_w_missing_meas} and \eqref{eq:luenberger_like_estimator} may be combined to define a dynamical system for the differences $\bar{x}_t = x_t - \hat{x}_t$, and the estimation error $\bar{z}_t = z_t - \hat{z}_t$:
\begin{subequations}
    \label{eq:estimation_error_system}
    \begin{align}
        \label{eq:estimation_error_system:xi}
            \bar{x}_{t+1} & = A \bar{x}_t + \estFeedback_t + w_t \\
            \errorOutput_t & =
                \begin{cases}
                    C \bar{x}_t + v_t, &  \modeSymbol^m_t = 1, \\
                    \emptyset, & \modeSymbol^m_t = 0.
                \end{cases}\label{eq:estimation_error_system:y}\\
            \bar{z}_t&=D\bar{x}_t.\label{eq:estimation_error_system:z}
    \end{align}
\end{subequations}

\begin{remark}\label{duality}
Equations \eqref{eq:affine_fb_law} and \eqref{eq:estimation_error_system} give \eqref{eq:system_w_missing_meas} and (\ref{eq:control_input}) under transformation
$$
B=I_{n_x},\; d=0_{n_z\times 1},\; \modeSymbol^c_t=1,\; x_t=\bar{x}_t,\; y_t=\bar{y}_t,\; z_t=\bar{z}_t,\; u_t=\estFeedback_t.
$$
Then, solving Problem \ref{prob:control_asap} with $N_c=T-1$ and ignoring the constraints $u_t\in\U$, gives an observer which keeps the estimation error $\bar{z}_t$ in $\performanceSet$ for all $t=0,\dots,T$, for all $x_0\in\X_0$, $w_t\in\W$, $v_t\in\V$. On the other hand, solving problem \ref{prob:control_alap} gives an observer which keeps the error $\bar{z}_t$ in $\performanceSet$ as long as possible, for all $x_0\in\X_0$, $w_t\in\W$, $v_t\in\V$. Note that in these cases, $\sigma^c_t$ are constants (equal to $1$) and not optimization variables. 
\end{remark}



==> sections/online.tex <==
In what we presented above, the optimization problem is solved offline, i.e., before any measurement is acquired. In this section, it is proposed that each time a measurement is received, the problem is solved again, but this time incorporating the information learned in the last measurement. We propose two methods to implement that.

First, We can use Lemma \ref{lem:hpoly_in_hpoly} to have a similar result when the interior polytope is defined by equalities instead of inequalities. In that case, such a polytope is an hyperplane.

\begin{corollary}[Hyperplane in H-Polytope]
\label{cor:hyperplane_in_hpoly}
Let $\mathbb{X} = \{ x \in \mathbb{R}^n \; | \; H_x x = h_x \}$, $\mathbb{Y} = \{ y \in \mathbb{R}^n \; | \; H_y y \leq h_y \} \subset \mathbb{R}^n$, $H_x \in \mathbb{R}^{q_x \times n}$, $H_y \in \mathbb{R}^{q_y \times n}$. We have $\mathbb{X} \subseteq \mathbb{Y}$ if and only if
    \begin{equation*}
        \exists \Lambda \in \mathbb{R}^{q_y \times q_x} \text{ such that }
        \Lambda H_x = H_y, \; \Lambda h_x \leq h_y.
    \end{equation*}
\end{corollary}
\begin{proof}
The structure of the proof consists in putting $\mathbb{X}$ in H-representation and applying Lemma \ref{lem:hpoly_in_hpoly}. One can write $\mathbb{X}=\{ x \in \mathbb{R} \; | \; \begin{bmatrix} H_x^\top & -H_x^\top \end{bmatrix}^\top x\leq\begin{bmatrix} h_x^\top & -h_x^\top \end{bmatrix}^\top \}$. Then, from Lemma \ref{lem:hpoly_in_hpoly}, $\mathbb{X}\subseteq\mathbb{Y}$ if and only if
\begin{equation*}
\exists \tilde{\Lambda} \in \mathbb{R}^{q_y \times 2q_x}_+ \text{ such that }
        \tilde{\Lambda} \begin{bmatrix} H_x\\ -H_x \end{bmatrix} = H_y, \; \tilde{\Lambda} \begin{bmatrix} h_x\\ -h_x \end{bmatrix} \leq h_y.
\end{equation*}
By decomposing $\tilde{\Lambda}=\begin{bmatrix} \Lambda_1 & \Lambda_2 \end{bmatrix}$ with $\Lambda_i\in\mathbb{R}^{q_y\times q_x}_+$ for $i\in\{1,2\}$, we have
\begin{align*}
\tilde{\Lambda}\begin{bmatrix} H_x\\ -H_x \end{bmatrix}= \begin{bmatrix} \Lambda_1 & \Lambda_2 \end{bmatrix} \begin{bmatrix} H_x\\ -H_x \end{bmatrix}=(\Lambda_1-\Lambda_2)H_x = \Lambda H_x,\\
\tilde{\Lambda}\begin{bmatrix} h_x\\ -h_x \end{bmatrix} = \begin{bmatrix} \Lambda_1 & \Lambda_2 \end{bmatrix}\begin{bmatrix} h_x\\ -h_x \end{bmatrix}=(\Lambda_1-\Lambda_2)h_x = \Lambda h_x,
\end{align*}
where $\Lambda\coloneqq\Lambda_1-\Lambda_2\in\R^{q_y \times q_x}$.
\end{proof}
\AA{Maybe it's too simple to put the proof. We can put a sketch of the proof instead. What do you think Kwesi?}

\KR{I think it is fair to assume that the reader knows
$$
H_x x = h_x \iff \begin{bmatrix} H_x \\ -H_x \end{bmatrix} x \leq \begin{bmatrix} h_x \\ -h_x \end{bmatrix},
$$
and so we do not need this corollary. Good work, though! 
}

\subsubsection{From last measurement (Fourier-Motzkin)}
Let's write $t_1$ the first measurement time, i.e., $t_1=\arg\min_t t$ such that $\modeSymbol^m_t=1$. We write $\X_{t_1}$ the set of possible values of $x_{t_1}$ knowing $y_{t_1}$. This set $\X_{t_1}$ will be considered as the new $\X_0$ and the problem will be solved again from this measurement. We can apply this iteratively.


First, we will see that $\X_{t_1}$ is a polytope and we will propose a method to compute a $H$-representation, i.e., a matrix $H_{\X_{t_1}}$ and a vector $h_{\X_{t_1}}$ such that
$$
\X_{t_1}=\{x_{t_1} | H_{\X_{t_1}} x_{t_1} \leq  h_{\X_{t_1}}\}.
$$
We are looking for the set of $x_{t_1}$ satisfying
\begin{align}
x_{t_1} &= R_{t_1} x \label{eq:new_initial_set:1}\\
x&=P_{x,:}\eta+\tilde{x} \label{eq:new_initial_set:2}\\
H_\eta\eta &\leq h_\eta \label{eq:new_initial_set:3}\\
y_{t_1} &= Cx_{t_1}+v_{t_1}, \label{eq:new_initial_set:4}
\end{align}
where $y_{t_1}$ is known. Equations (\ref{eq:new_initial_set:1}) and (\ref{eq:new_initial_set:2}) can be rewritten
$$
\begin{array}{lrcl}
& x_{t_1} &=& R_{t_1} ( P_{x,:}\eta+\tilde{x} )\\
\Leftrightarrow& x_{t_1}-R_{t_1}P_{x,:}\eta &=& R_{t_1}\tilde{x}\\
\Leftrightarrow& \begin{bmatrix}I & -R_{t_1}P_{x,:} \end{bmatrix}\begin{bmatrix} x_{t_1}\\ \eta \end{bmatrix}&=&R_{t_1}\tilde{x}\\
\Leftrightarrow& \begin{bmatrix}I & -R_{t_1}P_{x,:}\\ -I & R_{t_1}P_{x,:} \end{bmatrix}\begin{bmatrix} x_{t_1}\\ \eta \end{bmatrix}&\leq& \begin{bmatrix} R_{t_1}\tilde{x} \\ -R_{t_1}\tilde{x} \end{bmatrix}.
\end{array}
$$
Equation (\ref{eq:new_initial_set:3}) can be rewritten
$$
\begin{bmatrix}0& H_\eta \end{bmatrix} \begin{bmatrix} x_{t_1}\\ \eta \end{bmatrix}\leq h_\eta.
$$
Introducing the projection matrix $R^v_{t_1}$ such that, $v_{t_1}=R^v_{t_1}\eta$, equation (\ref{eq:new_initial_set:4}) can be rewritten
$$
\begin{array}{lrcl}
& y_{t_1} &=& Cx_{t_1}+R^v_{t_1}\eta\\
\Leftrightarrow& \begin{bmatrix}C & R^v_{t_1} \end{bmatrix} \begin{bmatrix} x_{t_1}\\ \eta \end{bmatrix} &=& y_{t_1}\\
\Leftrightarrow& \begin{bmatrix}C & R^v_{t_1} \\ -C & -R^v_{t_1} \end{bmatrix} \begin{bmatrix} x_{t_1}\\ \eta \end{bmatrix} &\leq& \begin{bmatrix} y_{t_1}\\ -y_{t_1}\end{bmatrix}.
\end{array}
$$
Finally, equations (\ref{eq:new_initial_set:1}) to (\ref{eq:new_initial_set:4}) are equivalent to
$$
\begin{bmatrix}
I & -R_{t_1}P_{x,:} \\
-I & R_{t_1}P_{x,:} \\
0 & H_\eta \\
C & R^v_{t_1} \\
-C & -R^v_{t_1}
\end{bmatrix}
\begin{bmatrix}
x_{t_1}\\ \eta
\end{bmatrix}
\leq
\begin{bmatrix}
R_{t_1}\tilde{x} \\
-R_{t_1}\tilde{x} \\
h_\eta \\
y_{t_1}\\
-y_{t_1}
\end{bmatrix}.
$$
We can use Fourier-Motzkin elimination to eliminate variable $\eta$. It leads to $H_{\X_{t_1}}$ and $h_{\X_{t_1}}$.

\subsubsection{From the beginning}
Another option is to solve the problem from $t=0$ but to add constraints on $\X_0$, $\W_t$ and $\V_t$ to keep only the values compatible with the measurements already acquired. In addition, variables corresponding to decisions already taken in the past are no longer variables but are data of the problem.

Let's consider that we have observed $y_{t_1},\dots,y_{t_k}$. Then, for all $j=1,\dots,k$ one can write
$$
\begin{array}{lrcl}
& y_{t_j} &=& Cx_{t_j}+v_{t_j}\\
\Leftrightarrow& y_{t_j} &=& CR_{t_j}x + R^v_{t_j}\eta\\
\Leftrightarrow& y_{t_j} &=& CR_{t_j}(P_{x,:}\eta+\tilde{x}) + R^v_{t_j}\eta\\
\Leftrightarrow& \left( CR_{t_j}P_{x,:} + R^v_{t_j} \right)\eta &=& y_{t_j}-CR_{t_j}\tilde{x}\\
\Leftrightarrow& \begin{bmatrix} CR_{t_j}P_{x,:} + R^v_{t_j} \\ -CR_{t_j}P_{x,:} - R^v_{t_j} \end{bmatrix} \eta &\leq& \begin{bmatrix} y_{t_j}-CR_{t_j}\tilde{x} \\ -y_{t_j}+CR_{t_j}\tilde{x} \end{bmatrix}\\
\Leftrightarrow& H_{t_j}\eta &\leq& h_{t_j}.
\end{array}
$$
This corresponds to additional constraints on $\X_0$ and on the sets $\W_t$, $\V_t$ for $t\leq t_j$. 





==> sections/trajectories_old.tex <==
Consider the three vector equations: \AA{For now, it does not work when $B\neq I$.}
\begin{subequations}\label{eq:xiDynamics}
    \begin{align}
        x & = J x_0 + S(w+u)  \\
        y & = \bar{C} x + v \\
        u & = F y + f
    \end{align}
\end{subequations}
where
$$
\begin{array}{cc}
    x = \begin{bmatrix} x_0^\top & x_1^\top & \cdots & x_T^\top \end{bmatrix}^\top \in \R^{n(T+1)},
    & w = \begin{bmatrix} w_0^\top & w_1^\top & \cdots & w_{T-1}^\top \end{bmatrix}^\top \in \R^{nT}, \\
    u = \begin{bmatrix} u_0^\top & u_1^\top & \cdots & u_{T-1}^\top \end{bmatrix}^\top \in \R^{nT},
    & y = \begin{bmatrix} y_0^\top & y_1^\top & \cdots & y_{T-1}^\top \end{bmatrix}^\top \in \R^{pT}, \\
    v = \begin{bmatrix} v_0^\top & v_1^\top & \cdots & v_{T-1}^\top \end{bmatrix}^\top \in \R^{pT},
    & f = \begin{bmatrix} f_0^\top & f_1^\top & \cdots & f_{T-1}^\top \end{bmatrix}^\top \in \R^{mT}, \\
\end{array}
$$
$$
J = 
\begin{bmatrix}
    I \\ A \\ A^2 \\ \vdots \\ A^{T-1}    
\end{bmatrix} \in \R^{n(T+1) \times n}, \;
S = 
\begin{bmatrix}
    0 & 0 & 0 & \cdots & 0 \\
    I & 0 & 0 & \cdots & 0 \\
    A & I & 0 & \cdots & 0 \\
    \vdots & \vdots & \vdots & \ddots & \\
    A^{T-1} & A^{T-2} & A^{T-3} & \cdots & I
\end{bmatrix}
\in \R^{n(T+1) \times nT}
$$
$$
\bar{C} = I_T \otimes C
$$
\AA{Is the definition of $\bar{C}$ correct?}
$$
F = 
\begin{bmatrix}
    F_{(0,0)} & 0 & 0 & \cdots & 0 \\
    F_{(1,0)} & F_{(1,1)} & 0 & \cdots & 0 \\
    \vdots & \vdots & \cdots & \ddots & \vdots \\
    F_{(T-1,0)} & F_{(T-1,1)} & F_{(T-1,1)} & \cdots & F_{(T-1,T-1)} \\
\end{bmatrix} \in \R^{mT \times pT}.
$$

The vector $x$ is the trajectory of the state and can be written as follows in terms of the disturbances and the initial state values: \AA{Should we develop ? If necessary, we have a development in the other document.}

\begin{equation}
  \label{eq:closed_loop_est_error}
  \left[ 
  \begin{array}{c}
      x	\\	u
  \end{array}
  \right]
  =
  \bar{P}
  \left[ 
  \begin{array}{c}
     w	\\	v
  \end{array}
  \right]
  +
  \left[ 
  \begin{array}{c}
      \tilde{x}	\\	\tilde{u}
  \end{array}
  \right],
\end{equation}
where
$$
\bar{P} = 
\left[ 
	\begin{array}{rl}
		P_{x w}	&	P_{x v} \\
        P_{u w}	&	P_{u v}
	\end{array}
\right],
$$
$$
\begin{array}{rlrl}
	P_{x w} = & S + SF(I-\bar{C} SF)^{-1} \bar{C} S, &
    P_{x v} = & SF(I-\bar{C} SF)^{-1}, \\
    P_{u w} = & F(I-\bar{C} SF)^{-1} \bar{C} S, &
    P_{u v} = & F(I - \bar{C} SF)^{-1},
\end{array}
$$
and 
$$
\begin{array}{rl}
	\tilde{x} = & Jx_0 + Sf + SF(I-\bar{C} SF)^{-1} ( \bar{C} Jx_0 + \bar{C} Sf ), \\
    \tilde{u} = & F(I-\bar{C} SF)^{-1} ( \bar{C} J x_0 + \bar{C} S f ) + f.
\end{array}
$$
